Generation and Transfer of Polarized Radiation in Hydrodynamical Models of the Solar Chromosphere

The main goal of this thesis has been to investigate the effects that the macroscopic vertical velocity fields have on the scattering polarization signals formed in the solar chromosphere. Until now, the impact of macroscopic motions had never been considered in the treatment of the polarization signals produced by scattering processes and the Hanle effect. This is especially important in the quiet solar chromosphere, given its strong dynamism and reduced magnetic field intensity. Our investigation focused in the solution of the multilevel, non-LTE radiative problem of the generation and transfer of polarized radiation in increasingly realistic atmosphere models (Milne-Eddington and two-level atom atmospheres, semi-empirical models with ad-hoc velocities, hydrodynamical time-dependent models and a snapshot of a 3D MHD simulation) for the Ca II IR triplet lines (at 8498, 8542 and 8662 A). As a particular result, we obtained the first synthetic tomography of a model quiet chromosphere that includes maps of linear polarization dominated by the Hanle effect and of circular polarization dominated by the Zeeman effect. We also studied the relevance of dynamic and thermodynamic in the inference of the chromospheric magnetic field orientation taking into account the 90{\deg} and 180{\deg} ambiguities and showing how velocity and temperature gradients can affect the diagnostic process. We show that Solar-C and the European Solar Telescope should be able to capture the dynamic effects simulated in this thesis for the Ca II IR triplet lines. Namely, the vertical velocity gradients are able to modulate the resulting scattering polarization amplitudes, specially in the presence of shock waves.

==> logoiac.tex <==
\begin{center}
 \begin{figure}[H]
  \begin{minipage}{\textwidth}
   \centering
%  \includegraphics[width=0.22\txw,height=0.15\txh]{fig_logoiac}  
   \includegraphics[scale=0.7]{fig_logoiac}  
   %\figcaption{\small \emph{}}
   %\label{fig:iac}
   %\vspace{0.35cm}
  \end{minipage}
 \end{figure}
\end{center}



==> logoull.tex <==
\begin{center}
 \begin{figure}[H]
  \begin{minipage}{\textwidth}
   \centering
   \includegraphics[scale=0.4]{fig_logoull}  
   %\figcaption{\small \emph{}}
   %\label{fig:ull}
   %\vspace{0.35cm}
  \end{minipage}
 \end{figure}
\end{center}


